AxFormer: Accuracy-driven Approximation of Transformers for Faster, Smaller and more Accurate NLP Models

Transformers have greatly advanced the state-of-the-art in Natural Language Processing (NLP) in recent years, but present very large computation and storage requirements. We observe that the design process of Transformers (pre-train a foundation model on a large dataset in a self-supervised manner, and subsequently fine-tune it for different downstream tasks) leads to task-specific models that are highly over-parameterized, adversely impacting both accuracy and inference efficiency. We propose AxFormer, a systematic framework that applies accuracy-driven approximations to create optimized transformer models for a given downstream task. AxFormer combines two key optimizations -- accuracy-driven pruning and selective hard attention. Accuracy-driven pruning identifies and removes parts of the fine-tuned transformer that hinder performance on the given downstream task. Sparse hard-attention optimizes attention blocks in selected layers by eliminating irrelevant word aggregations, thereby helping the model focus only on the relevant parts of the input. In effect, AxFormer leads to models that are more accurate, while also being faster and smaller. Our experiments on GLUE and SQUAD tasks show that AxFormer models are up to 4.5% more accurate, while also being up to 2.5X faster and up to 3.2X smaller than conventional fine-tuned models. In addition, we demonstrate that AxFormer can be combined with previous efforts such as distillation or quantization to achieve further efficiency gains.

==> Sections/preliminaries.tex <==
\begin{figure*}[htbp]
\centerline{\includegraphics[width=\textwidth,height=5cm]{Figures/Picture41.png}}
\caption{\textbf{A typical Transformer architecture and its elements.} At fine-tuning time, a task-specific final layer is added to the pre-trained model and trained. Specialization identifies and removes harmful elements from the fine-tuned model, and modifies the attention mechanism in selected layers. Specialized models are smaller, faster, more energy-efficient and more accurate than the conventional fine-tuned models.}
\label{fig:background}
\end{figure*}

A Transformer (Fig.~\ref{fig:background}) consists of an embedding layer, followed by multiple transformer layers stacked together, and a task-specific final layer. A transformer layer consists of the multi-headed self-attention operation (ATTN block), followed by a feed-forward neural network (FFN block) with layer norm operations at the input and output of the layer. In this work, we define the {\em elements} of a Transformer to include different levels of granularity, {\em i.e.}, ATTN blocks, FFN blocks, Attention Heads and Neurons. The core of the Transformer is the ATTN block that builds representations based on the extent of attention (dot product of embedding vectors) each token in the input sequence places on every other token in the sequence. This operation, called self-attention, helps Transformers capture and understand the structure of language during pre-training, thereby enabling state-of-the-art performance in the different downstream tasks after fine-tuning.

Prior research \cite{DBLP:conf/acl/JawaharSS19} has explored how Transformers learn to understand language during training. It was found that BERT captures phrase-level information in the lower layers, mapping related tokens together. The lower layers also capture surface features, while the middle layers capture syntatic features and higher layers capture semantic features. It was also observed that BERT requires deeper layers only when long-range dependency information is required. We utilize these insights in our work to guide the Specialization process, since different downstream tasks require different types of linguistic knowledge, and hence, different elements in the Transformer become harmful or redundant.




